Towards an Achievable Performance for the Loop Nests

Numerous code optimization techniques, including loop nest optimizations, have been developed over the last four decades. Loop optimization techniques transform loop nests to improve the performance of the code on a target architecture, including exposing parallelism. Finding and evaluating an optimal, semantic-preserving sequence of transformations is a complex problem. The sequence is guided using heuristics and/or analytical models and there is no way of knowing how close it gets to optimal performance or if there is any headroom for improvement. This paper makes two contributions. First, it uses a comparative analysis of loop optimizations/transformations across multiple compilers to determine how much headroom may exist for each compiler. And second, it presents an approach to characterize the loop nests based on their hardware performance counter values and a Machine Learning approach that predicts which compiler will generate the fastest code for a loop nest. The prediction is made for both auto-vectorized, serial compilation and for auto-parallelization. The results show that the headroom for state-of-the-art compilers ranges from 1.10x to 1.42x for the serial code and from 1.30x to 1.71x for the auto-parallelized code. These results are based on the Machine Learning predictions.

==> approach.tex <==
\section{Approach} \label{sec:approach}
This section describes our methodology for collecting code for the loop nests and later profiling them to collect the hardware performance counters.
These hardware performance counters then function as the \textit{features} to the Machine Learning models.
%
\subsection{Loop Extraction}
This work focuses on the loop nests since loop nests dominate the performance in various applications.
Therefore, the \texttt{for} loops are extracted from various \texttt{C} benchmarks.
%, to collect data about their performance and their hardware performance counters values.
Our extractor is based on the loop extractor implemented by Chen et. al.\cite{Chen17}.
The loop extractor is implemented using the \texttt{ROSE} source-to-source compiler infrastructure\cite{Quinlan00} and operates on C applications, one of the most widely used languages for High-Performance Computing.
The extractor instruments code to record the performance data for the loop nests without making any modifications to the loop iteration count or loop body. 
%Therefore, the code optimizers' behavior remains virtually consistent regarding the loop transformations even after the extraction from the original source code. 
%Loops with a negligible execution time are omitted.
Readers interested in the technical details about the implementation of the loop extractor can refer to the previously mentioned work by Chen et. al.
%
\subsection{Collecting Hardware Performance Counters using Profiling}
The features, i.e., the hardware performance counters used for the Machine Learning (ML) models are collected by profiling loop nests using Intel's VTune Amplifier.   
We use generated code from Intel's ICC compiler to generate the executable that is then used for profiling.
All the loop optimizations are disabled during this compilation by using the -O1 flag.
In addition to that, the optimization that are responsible for vector code generation and parallel code generation are disabled too.
The profiling information, therefore, provides an insight into the characteristics of the loop nests while eliminating the influence of compiler transformations and behavioral changes incurred from special architectural features of the underlying architecture.
The performance counters that are collected include instruction-based (instruction types and counts), CPU clock cycles-based (including stalls), memory-based (D-TLB, L1 cache, L2 cache, L3 cache).

Once the hardware performance counters are collected for the loop nests, we skip dynamic instruction count as a feature and normalize the rest of the hardware performance counters in terms of \textit{per kilo instructions} (PKI).
Based on our analysis, this allows the Machine Learning models to learn about the inherent characteristics of the loop nests and not bias them towards characteristics such as loop trip count.
%\note{Instruction Count as a separate feature after normalization?}
%
\subsection{Most Suited Code Optimizer}
To train the ML models, each feature vector needs to be correlated with a \textit{target} class. Since in this work we are focusing on hardware performance counters as features to predict a code optimizer, we are using \textit{Classification} algorithms for which code optimizer is the target class.

To create the dataset, we optimize the loop nests with the candidate code optimizers and then execute them to record their performance in terms of wall clock time. 
The code optimizers are configured to optimize the loop nests for the underlying architectures for which we train the ML models.
These optimizations include the loop transformations and code generation optimizations for the specific architectures. 
For serial code experiments, transformations for auto-vectorization are enabled.
Whereas, for parallel code experiments, transformations for auto-vectorization and auto-parallelization are enabled.

The most suited candidate for a loop nest on a particular architecture, i.e., the code optimizer that produces the best performing code for the loop nests, is appended in the dataset as the target class for that specific loop nest. The feature vector in the dataset remains same across all experiments, just the target class differs based on the architecture we are making predictions for and the purpose of the classifier.
%NOT THIS PAPER - Saving this cost of executing optimized loop nests multiple times - at least once for each available code optimizers - to find the best code optimizer is the focus of this work.    
%
\subsection{Machine Learning Model Setup}\label{section:ML_setup}
%
%\begin{figure}[ht]
%\centering
%\input{figs/ML_setup}
%\caption{Training Machine Learning model using Hardware Performance Counters}
%\label{fig:ML_setup}
%\end{figure}
%
\subsubsection{Random Decision Forest Classifier (RF)}
We chose Random Decision Forest\cite{Ho95} as our classification algorithm to predict the optimal compiler for the loop nests. RF is a learning algorithm that builds on the principles behind Decision Trees.
% regression problems as well as unsupervised learning among others.
Generally, the Decision Tree algorithm, learns from training data by building a structured and hierarchical representation of the correlation between features and classes.
Features represent the nodes in the trees and classes are leaves at the deepest level.
An optimal Decision Tree would perfectly and accurately divide the data among the target classes.
However, finding an optimal tree is an NP-Complete problem, therefore we have to rely on heuristics such as greedy search.

% With this in mind, a typical Decision Tree algorithm would proceed as follows. Choose the feature that has the highest Information Gain Ratio in relation to the training dataset.
% That is, the feature that separates the highest number of instances of a specific class.
% Use that feature as the first decision node.
% If no feature is found that makes for a perfect separation (where instances of another target are not found), then choose the one that minimizes the presence of instances from another target value.
% Based on the separation created by the first node, re-evaluate the Information Gain Ratio of the remaining features and choose the best one for next decision node.
% When the first feature didn't create a perfect separation, this has to be repeated for every leaf created by the first node.
% Repeat step 2 until a perfect separation of classes is achieved in every leaf or a threshold is fulfilled.
% Classification is done by following the decision nodes according to the features of the testing data.
%
Decision Trees suffer from several issues.
The main one being a tendency towards overfitting, that is, the tree loses generalization the deeper the tree goes, modeling the trend for training data but be inaccurate for new instances.
RF provides a better solution for overfitting and classification bias by adding two stochastic steps to the Decision Tree Algorithm.
% This is a general description of a Random Forest algorithm:
From the training dataset, RF creates a bootstrapped subset by stochastically choosing the instances or features (with repeats allowed) that will be used for building the decision trees.
This is called Bootstrap Aggregating (bagging for short) and the instances inside the created subset are called In-Bag instances.
After creating the Bagged dataset, an arbitrary number of decision trees are built using subsets of randomly chosen features.
The depth of the trees is limited by the number of features allowed (according to a predetermined threshold) and by another arbitrary number.
Each decision tree accuracy is evaluated using the remaining (out-of-bag) instances that weren't part of the Decision Tree building phase.

Classification is achieved through a voting algorithm, where a target value is generated by each Random Tree, the one with the highest number of trees will be the class assigned to the new instance.

Since Random Forest is constantly evaluating the performance of the subsets of features, we can easily detect the ones that were used in the better performing trees. 
Therefore, we require little to no feature filtering before running the algorithm.
This is useful when approaching a new problem where the correlation between the input features and the output class is not entirely known.

%
\subsection{Machine Learning Model Configurations}
We partition the dataset, or the loop repository, to create a training dataset and a validation dataset.  
The training dataset allows us to train and tune the ML models.
We evaluate our trained models on Accuracy and Area Under Curve (AUC).
Whereas, the validation is a set of unseen loop nests that we use to make predictions.
The results reported in the following sections in regards to the performance of the ML predictions as based on the loops from the validation dataset.
Fig. \ref{fig:ML_setup} shows the overall setup to make predictions about the code optimizer for the loop nests.
%
\subsubsection{Serial Code}
The dataset consists of hardware performance counters values for the loops and the most suited optimizer for an architecture as the target.
Later, we train the multi-class RF classifier to make the predictions. 
Majority Classifier serves as the baseline to evaluate the trained model. 
Majority Classifier is a feature-agnostic classifier that determines the output for every instance to be equal to the target that has most instances in the training set.
%
\subsubsection{Auto-Parallelized Code}
In this case, the dataset uses the same set of hardware performance counters as those used to predict the most suited serial code optimizer.
Again, Majority Classifier serves as the baseline.
We train two models for auto-parallelized code. In each case the features remain the same, just the target varies based on the purpose of the ML model.

The first model predicts the most suited code optimizer for the loop using a multi-class RF classifier.
Therefore, for the dataset the target is the optimizer that produces the best performing auto-parallelized code for the loop nests.
The next model uses a binary RF classifier to predict if the performance benefits will be \textit{profitable} by having a parallel execution instead of the serial execution.
If any of the candidate optimizers were able to parallelize the serial code with at least 5\% speedup, we deem the loop as \textit{profitable} i.e. the target is YES, otherwise NO. 
If any candidate code optimizer was able to auto-parallelize a loop nest with at least 5\% speedup, we put the target as YES in the ML dataset.
%The third model predicts the number of threads that will produce the best performance for the loop nest.
%In this case, the target for the dataset is most suited number of threads and the classifier is a multi-class RF classifier.
%For example, the targets for a multi-core processor that can process 64 threads would be: serial (1 thread), half of the available parallelism (32 threads) and maximum parallelism (64 threads). 
%This model aims for the potential for scalability, data movement cost and the burden on processor resources such local and shared memory. 

These models together are expected to determine the most suited optimizer for the loop nest and thereafter if running the loop sequentially might save resources without hampering the performance.


==> related_work.tex <==
\section{Related Work} \label{sec:priorart}
Prior works that have addressed challenges in compiler optimizations using Machine Learning have focused on auto-vectorization\cite{Stock12,Watkinson17} and on scalability and scheduling configurations for the parallelism\cite{Barnes08,Wang09,Tournavitis09}.

Stock et. al.\cite{Stock12} developed a ML-based performance model to guide SIMD compiler optimizations for vectorizing tensor contraction computations.
However in this work, we explore kernels from a variety of computations to predict an optimizer than can generate an efficient serial code, which includes auto-vectorized code.
Watkinson et. al.\cite{Watkinson17} in their work use ML models to predict opportunities for auto-vectorization and its profitability across multiple compilers and architectures.
They also predict opportunities for manual vectorization in loop nests that were not auto-vectorized by the compilers.
In this work, we too explore multiple code optimizers and architectures, but we are not concerned with performance gains just related to vector code generation.
Like this work, they too use just the dynamic features to train ML models but they collect hardware performance counters separately for each architecture to make predictions. 

Tournavitis et. al.\cite{Tournavitis09} use a mix of static and dynamic features to develop a platform-agnostic, profiling-based parallelism detection method for sequential applications. 
Their method requires user's approval for parallelization decisions that cannot be proven conclusively.
They use ML models to judge the profitability on parallelization and to select the scheduling policy.
In contrast, our work uses just the dynamic features to train ML models and we let the ML models choose the most suited candidate that can generate a profitable auto-parallelized code. 
In the work by Wang et. al.\cite{Wang09}, they predicted fine-grain parallelism mappings of OpenMP programs.
Their ML models predicted optimal number of threads and the optimal scheduling policy using a mix of static and dynamic features.
Similar to their work, we also treat loop nests from different datasets as different entities.
In our work, we start with serial code instead of OpenMP parallelized code and we can't control the scheduling policy for every auto-parallelization optimizer, therefore we chose to do experiments with the default settings of the code optimizers.


==> summary.tex <==
\section{Conclusions} \label{sec:conclusion}
In this work we explored the possibility of predicting a code optimizer for the loop nests solely based on their inherent behavior that can be detected from the hardware performance counters.
We show that Machine Learning algorithms can predict the most suited serial code and auto-parallelized code optimizer for the loop nests.
In addition to that, the models can predict the profitability of executing a parallel version of the loop nest on a specific architecture so as to save resources without losing performance.
We have also shown that the hardware performance counters from an architecture can also be used to make predictions for a similar architecture.

Even though the code optimizers have the capability of performing similar set of loop transformation techniques, they can produce optimized versions of the code that have significant difference in performance.
This shows that state-of-the-art code optimizers miss out on opportunities for producing efficient code and our approach can help towards identifying those opportunities and making improvements in order to achieve better performance. 

